Quickest Detection and Forecast of Pandemic Outbreaks: Analysis of COVID-19 Waves

The COVID-19 pandemic has, worldwide and up to December 2020, caused over 1.7 million deaths, and put the world's most advanced healthcare systems under heavy stress. In many countries, drastic restrictive measures adopted by political authorities, such as national lockdowns, have not prevented the outbreak of new pandemic's waves. In this article, we propose an integrated detection-estimation-forecasting framework that, using publicly available data, is designed to: (i) learn relevant features of the pandemic (e.g., the infection rate); (ii) detect as quickly as possible the onset (or the termination) of an exponential growth of the contagion; and (iii) reliably forecast the pandemic evolution. The proposed solution is validated by analyzing the COVID-19 second and third waves in the USA.

==> figures/beta-v4.tex <==
\newcommand{\commonScale}{.72}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-14mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{14mm}{\hspace{0mm}{Infection Rate}}}
%
\newcommand{\legendScale}{.65}
%
\psfrag{leg1}[l][l]	[\legendScale]{	\raisebox{-3mm}{\hspace{-2mm}{Bayesian Learning (all data)}}}
\psfrag{leg2}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Forecast A (No restriction)}}}
\psfrag{leg3}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Forecast B (With restriction)}}}
%
\newcommand{\xscale}{.60}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-4mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff 01-May}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff 29-May}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff 26-Jun}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff 24-Jul}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff 21-Aug}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff 18-Sep}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff 16-Oct}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff 13-Nov}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff 11-Dec}}
%
%
\newcommand{\yscale}{.60}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $.005$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $.010$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $.015$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $.020$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $.025$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $.030$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $.035$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $.040$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $.045$}}
\psfrag{y11}[r][r]	[\yscale]{	\yvoff{\yhoff $.050$}}

==> figures/block-diagram-v14.tex <==
\definecolor{redCustom}{RGB}{200,0,0}
\definecolor{greenCustom}{RGB}{0,200,0}

\psfrag{obs}[c][c]	[.45]{	\raisebox{-3mm}{\hspace{0mm}{Continue Observing}}}

\psfrag{td}[c][c]	[.65]{	\raisebox{-6mm}{\hspace{0mm}{\textsc{Today}}}}

\psfrag{t1}[c][c]	[.8]{	\raisebox{-10mm}{\hspace{0mm}{\textsc{Input Data}}}}
\psfrag{t2}[c][c]	[.8]{	\raisebox{-10mm}{\hspace{0mm}{\textsc{Pre-Processing}}}}
\psfrag{t3}[c][c]	[.8]{	\raisebox{-8mm}{\hspace{0mm}{\textsc{Bayesian Learning}}}}
\psfrag{t4}[c][c]	[.8]{	\raisebox{-8mm}{\hspace{0mm}{\textsc{Parameters Forecast}}}}
\psfrag{t5}[c][c]	[.8]{	\raisebox{-10mm}{\hspace{0mm}{\textsc{Growth Rate}}}}
\psfrag{t6}[c][c]	[.8]{	\raisebox{-8mm}{\hspace{0mm}{\textsc{Quickest Detection}}}}
\psfrag{t7}[c][c]	[.8]{	\raisebox{-8mm}{\hspace{0mm}{\textsc{Pandemic Forecast}}}}

\psfrag{tb11}[l][l]	[.7]{	\raisebox{0mm}{\hspace{0mm}{\textit{Publicly available data (such as}}}}
\psfrag{tb12}[l][l]	[.7]{	\raisebox{0mm}{\hspace{0mm}{\textit{positive and recovered individuals)}}}}
\psfrag{tb13}[l][l]	[.7]{	\raisebox{0mm}{\hspace{0mm}{\textit{are collected daily.}}}}

%% \psfrag{tb21}[l][l]	[.7]{	\raisebox{0mm}{\hspace{0mm}{\textit{The sequence of daily new}}}}
%% \psfrag{tb22}[l][l]	[.7]{	\raisebox{0mm}{\hspace{0mm}{\textit{positives is pre-processed to}}}}
%% \psfrag{tb23}[l][l]	[.7]{	\raisebox{0mm}{\hspace{0mm}{\textit{mitigate gross errors and weekly}}}}
%% \psfrag{tb24}[l][l]	[.7]{	\raisebox{0mm}{\hspace{0mm}{\textit{fluctuations.}}}}

\psfrag{c1}[c][c]	[.75]{	\raisebox{1mm}{\hspace{5mm}{Onset of 1st Wave}}}
\psfrag{c2}[c][c]	[.75]{	\raisebox{-2mm}{\hspace{0mm}{End of 1st Wave}}}
\psfrag{c3}[c][c]	[.75]{	\raisebox{0mm}{\hspace{5mm}{Onset of 2nd Wave}}}

\psfrag{d1}[c][c]	[.65]{	\raisebox{0mm}{\hspace{0mm}{1st Wave}}}
\psfrag{d2}[c][c]	[.65]{	\raisebox{0mm}{\hspace{0mm}{End 1st Wave}}}
\psfrag{d3}[c][c]	[.65]{	\raisebox{0mm}{\hspace{0mm}{2nd Wave}}}

\psfrag{e1}[c][c]	[.65]{	\raisebox{0mm}{\hspace{0mm}{Confidence}}}
\psfrag{e2}[c][c]	[.65]{	\raisebox{0mm}{\hspace{0mm}{Interval}}}
\psfrag{e3}[c][c]	[.65]{	\raisebox{0mm}{\hspace{0mm}{Confidence Interval}}}

%% \psfrag{tb31}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{Epidemiological model's parameters are}}}}
%% \psfrag{tb32}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{sequentially learned through the input data.}}}}

\psfrag{tb31}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{Learning is based on epidemiological}}}}
\psfrag{tb32}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{compartmental models (e.g., SIR). Model}}}}
\psfrag{tb33}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{states (S,I,R) and parameters ($\beta$ and $\gamma$) are}}}}
\psfrag{tb34}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{sequentially learned from the data.}}}}

\psfrag{tb41}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{The output of the ``quickest detection'' controls the}}}}
\psfrag{tb42}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{parameters and pandemic  forecast. If in critical regime,}}}}
\psfrag{tb43}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{the infection rate is expected to increase, as well as the}}}}
\psfrag{tb44}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{number of infected; on the other hand, if in controlled }}}}
\psfrag{tb45}[l][l]	[.7]{	\raisebox{10mm}{\hspace{0mm}{\textit{regime, infection rate is  expected to decrease.}}}}


\psfrag{tb51}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{The pandemic growth rate is}}}}
\psfrag{tb52}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{computed as the ratio between two}}}}
\psfrag{tb53}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{consecutive daily positive case}}}}
\psfrag{tb54}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{counts. When growth rate > 1,}}}}
\psfrag{tb55}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{the pandemic is in a critical}}}}
\psfrag{tb56}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{regime; otherwise,  it is in a}}}}
\psfrag{tb57}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{controlled regime. Clearly, the}}}}
\psfrag{tb58}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{growth rate is randomly fluctuating,}}}}
\psfrag{tb59}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{thus requiring the design of}}}}
\psfrag{tb50}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{a proper statistical test.}}}}

\psfrag{tb61}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{MAST statistics are used to detect the onset and }}}}
\psfrag{tb62}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{termination of pandemic waves, namely, the}}}}
\psfrag{tb63}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{beginning of critical or controlled regimes. In}}}}
\psfrag{tb64}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{the above example as of \textsc{Today}, the pandemic}}}}
\psfrag{tb65}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{is in a critical regime.}}}}
%% \psfrag{tb66}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{}}}}

\psfrag{tb71}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{The forecasted model's parameters are used to predict }}}}
\psfrag{tb72}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{the evolution of the pandemic.}}}}
%% \psfrag{tb73}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{}}}}
%% \psfrag{tb74}[l][l]	[.7]{	\raisebox{-10mm}{\hspace{0mm}{\textit{}}}}

\psfrag{leg1}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-2mm}{Daily new positives}}}
\psfrag{leg2}[l][l]	[.65]{	\raisebox{0mm}{\hspace{-2mm}{Recovered}}}

\psfrag{uno}[c][c]	[.75]{	\raisebox{0mm}{\hspace{-1mm}{$1$}}}

\psfrag{thr}[c][c]	[.75]{	\raisebox{0mm}{\hspace{0mm}{Thr.}}}

\psfrag{b1}[c][c]	[.9]{	\raisebox{0mm}{\hspace{-1.3mm}{S}}}
\psfrag{b2}[c][c]	[.9]{	\raisebox{0mm}{\hspace{-1.3mm}{I}}}
\psfrag{b3}[c][c]	[.9]{	\raisebox{0mm}{\hspace{-1.3mm}{R}}}

\psfrag{st3}[c][c]	[.75]{	\raisebox{4mm}{\hspace{0mm}{Infection Rate}}}
\psfrag{st4}[c][c]	[.75]{	\raisebox{4mm}{\hspace{0mm}{Recovery Rate}}}

\psfrag{be}[c][c]	[.9]{	\raisebox{-4mm}{\hspace{-1mm}{\textcolor{redCustom}{$\beta$}}}}
\psfrag{ga}[c][c]	[.9]{	\raisebox{-4mm}{\hspace{-1mm}{\textcolor{greenCustom}{$\gamma$}}}}
\psfrag{be2}[c][c]	[.9]{	\raisebox{20mm}{\hspace{0mm}{\textcolor{redCustom}{$\beta$}}}}
\psfrag{ga2}[c][c]	[.9]{	\raisebox{18mm}{\hspace{0mm}{\textcolor{greenCustom}{$\gamma$}}}}

\psfrag{st1}[c][c]	[.75]{	\raisebox{4mm}{\hspace{0mm}{Controlled Regime}}}
\psfrag{st2}[c][c]	[.75]{	\raisebox{4mm}{\hspace{0mm}{Critical Regime}}}

==> figures/data-v3.tex <==
\newcommand{\commonScale}{.72}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-14mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{6mm}{\hspace{0mm}{\# Individuals (in millions)}}}
\psfrag{yla2}[c][c]	[\commonScale]{	\raisebox{10mm}{\hspace{0mm}{\# Individuals (in thousands)}}}
%
\newcommand{\legendScale}{.65}
%
\psfrag{leg1}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-13mm}{Number of Infected}}}
\psfrag{leg2}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-13mm}{Number of Recovered}}}
\psfrag{leg3}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-13mm}{Number of Daily New Positives}}}
%
\newcommand{\xscale}{.60}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-4mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff 01-Mar}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff 05-Apr}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff 10-May}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff 14-Jun}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff 19-Jul}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff 23-Aug}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff 27-Sep}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff 01-Nov}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff 06-Dec}}
%
%
\newcommand{\yscale}{.60}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $1$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $2$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $3$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $4$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $5$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $6$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $7$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $8$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $9$}}
\psfrag{y11}[r][r]	[\yscale]{	\yvoff{\yhoff \color[rgb]{0,0.45,0.74} $10$}}
%
\psfrag{yr1}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $0$}}
\psfrag{yr2}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $20$}}
\psfrag{yr3}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $40$}}
\psfrag{yr4}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $60$}}
\psfrag{yr5}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $80$}}
\psfrag{yr6}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $100$}}
\psfrag{yr7}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $120$}}
\psfrag{yr8}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $140$}}
\psfrag{yr9}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $160$}}
\psfrag{yr10}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $180$}}
\psfrag{yr11}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $200$}}
\psfrag{yr12}[l][l]	[\yscale]{	\yvoff{\hspace{-2.5mm} \color[rgb]{0.85,0.33,0.10} $220$}}

==> figures/infected-053-v4.tex <==
\newcommand{\commonScale}{.72}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-14mm}{\hspace{0mm}{Date}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{6mm}{\hspace{0mm}{\# Individuals (in millions)}}}
%
\newcommand{\legendScale}{.65}
%
\psfrag{leg1}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Number of Infected}}}
\psfrag{leg2}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Forecast A (No restriction)}}}
\psfrag{leg3}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Forecast B (With restriction)}}}
%
\newcommand{\xscale}{.60}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-4mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff 01-May}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff 29-May}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff 26-Jun}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff 24-Jul}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff 21-Aug}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff 18-Sep}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff 16-Oct}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff 13-Nov}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff 11-Dec}}
%
%
\newcommand{\yscale}{.60}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $1$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $2$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $3$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $4$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $5$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $6$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $7$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $8$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $9$}}
\psfrag{y11}[r][r]	[\yscale]{	\yvoff{\yhoff $10$}}

==> figures/mast-v4-opt3.tex <==
\newcommand{\commonScale}{.72}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-14mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{8mm}{\hspace{0mm}{MAST Statistic}}}
%
\newcommand{\legendScale}{.65}
%
\psfrag{leg1}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Statistic for Onset Detection 2nd Wave}}}
\psfrag{leg2}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Statistic for Termination Detection 2nd Wave}}}
\psfrag{leg3}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Statistic for Onset Detection 3rd Wave}}}
\psfrag{leg4}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Statistic for Termination Detection 3rd Wave}}}
\psfrag{leg5}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Threshold}}}
%
\psfrag{sd0}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{1-May}}}
\psfrag{sd1}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-1.5mm}{22-Jun}}}
\psfrag{sd2}[l][l]	[\legendScale]{	\raisebox{-4mm}{\hspace{-1.5mm}{12-Aug}}}
\psfrag{sd3}[l][l]	[\legendScale]{	\raisebox{-4mm}{\hspace{-1.5mm}{29-Sep}}}
%
\newcommand{\xscale}{.60}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-4mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff 01-Mar}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff 05-Apr}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff 10-May}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff 14-Jun}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff 19-Jul}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff 23-Aug}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff 27-Sep}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff 01-Nov}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff 06-Dec}}
%
%
\newcommand{\yscale}{.60}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $1$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $2$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $3$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $4$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $5$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $6$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $7$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $8$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $9$}}
\psfrag{y11}[r][r]	[\yscale]{	\yvoff{\yhoff $10$}}

==> figures/performance-v5.tex <==
\newcommand{\commonScale}{.72}

\psfrag{xla}[c][c]	[\commonScale]{	\raisebox{-14mm}{\hspace{0mm}{Day of Forecasting}}}
\psfrag{yla}[c][c]	[\commonScale]{	\raisebox{10mm}{\hspace{0mm}{Mean Absolute Percentage Error}}}
%
\newcommand{\legendScale}{.65}
%
\psfrag{leg1}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Proposed, Strategy A - Horizon 4 Weeks}}}
\psfrag{leg2}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Proposed, Strategy B - Horizon 4 Weeks}}}
\psfrag{leg3}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{GSEIR-fit - Horizon 4 Weeks}}}
\psfrag{leg4}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Proposed, Strategy A - Horizon 2 Weeks}}}
\psfrag{leg5}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{Proposed, Strategy B - Horizon 2 Weeks}}}
\psfrag{leg6}[l][l]	[\legendScale]{	\raisebox{0mm}{\hspace{-2mm}{GSEIR-fit - Horizon 2 Weeks}}}
%
\newcommand{\xscale}{.60}
\newcommand{\xhoff}{\hspace{0mm}}
\newcommand{\xvoff}{\raisebox{-4mm}}
%
\psfrag{x1}[ct][ct]	[\xscale]{	\xvoff{\xhoff 01-May}}
\psfrag{x2}[ct][ct]	[\xscale]{	\xvoff{\xhoff 29-May}}
\psfrag{x3}[ct][ct]	[\xscale]{	\xvoff{\xhoff 26-Jun}}
\psfrag{x4}[ct][ct]	[\xscale]{	\xvoff{\xhoff 24-Jul}}
\psfrag{x5}[ct][ct]	[\xscale]{	\xvoff{\xhoff 21-Aug}}
\psfrag{x6}[ct][ct]	[\xscale]{	\xvoff{\xhoff 18-Sep}}
\psfrag{x7}[ct][ct]	[\xscale]{	\xvoff{\xhoff 16-Oct}}
\psfrag{x8}[ct][ct]	[\xscale]{	\xvoff{\xhoff 13-Nov}}
\psfrag{x9}[ct][ct]	[\xscale]{	\xvoff{\xhoff 11-Dec}}
%
%
\newcommand{\yscale}{.60}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $0$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $5$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $15$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $20$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $25$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $30$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $35$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $40$}}
